An efficient algorithm computing composition factors of $T(V)^{\otimes n}$

We present an algorithm that computes the composition factors of the n-th tensor power of the free associative algebra on a vector space. The composition factors admit a description in terms of certain coefficients $c_{\lambda\mu}$ determining their irreducible structure. By reinterpreting these coefficients as counting the number of ways to solve certain `decomposition-puzzles' we are able to design an efficient algorithm extending the range of computation by a factor of over 750. Furthermore, by visualising the data appropriately, we gain insights into the nature of the coefficients leading to the development of a new representation theoretic framework called PD-modules.

==> algorithms/mu_decompositions.tex <==
\begin{minipage}{.9\linewidth}

\begin{algorithm}[H]

\label{AlgMuDecompositions}

\SetKwFunction{MuDecompositions}{\textsc{mu$\_$decompositions}}

\BlankLine

\KwInput{A partition $\mu \vdash m$.}

\BlankLine

\KwResult{Return an hash table mapping shapes $\theta$ to their $\mu$-decompositions.}

\BlankLine

Initialise empty hash $\mathcal{M}$.

\BlankLine

\For{$\theta \vdash m$}{
Initialise empty array A[].

\BlankLine



}


\caption{$\mu$-Decompositions}


\end{algorithm}


\end{minipage}

==> figures/cf_display_side_by_side.tex <==
\begin{tikzpicture}[scale=2]

\node[anchor=north west, inner sep=0]
(image1) at (0,0) {\includegraphics[scale=0.135]{images/cf_display_5}};

\node[anchor=north west, inner sep=0]
(image2) at (0,-4.5) {\includegraphics[scale=0.24]{images/cf_display_14_clean}};

\end{tikzpicture}




==> figures/cf_rays.tex <==
\begin{tikzpicture}[scale=0.8]


\node[anchor=north west, inner sep=0]
(image) at (0,0) {\includegraphics[width=0.7\textwidth]{images/cf_display_14_no_bar}};


\coordinate (O) at (1.742,-1.395);
\coordinate (A) at (9.5, -12);

\draw[fill] (O) circle (0.05);
\draw (O) -- (A);












\end{tikzpicture}









